Transmission and Storage Rates for Sequential Massive Random Access

This paper introduces a new source coding paradigm called Sequential Massive Random Access (SMRA). In SMRA, a set of correlated sources is encoded once for all and stored on a server, and clients want to successively access to only a subset of the sources. Since the number of simultaneous clients can be huge, the server is only allowed to extract a bitstream from the stored data: no re-encoding can be performed before the transmission of the specific client's request. In this paper, we formally define the SMRA framework and introduce both storage and transmission rates to characterize the performance of SMRA. We derive achievable transmission and storage rates for lossless source coding of i.i.d. and non i.i.d. sources, and transmission and storage rates-distortion regions for Gaussian sources. We also show two practical implementations of SMRA systems based on rate-compatible LDPC codes. Both theoretical and experimental results demonstrate that SMRA systems can reach the same transmission rates as in traditional point to point source coding schemes, while having a reasonable overhead in terms of storage rate. These results constitute a breakthrough for many recent data transmission applications in which different parts of the data are requested by the clients.

==> rate-storage-generalization-mra.tex <==
% !TeX root = intercom.tex
%
\section{Optimal rate-storage bounds for MRA to discrete i.i.d. sources}
\label{sec:RSboundsMRA:iid}
Section~\ref{sec:RSbounds:iid} studies Sequential MRA and considers that only the previous requested source is held in memory at the decoder (see Theorem~\ref{th:iid_stat_known} and Definition~\ref{def:MRA}). This Section generalizes these results in two directions. First, Lemma~\ref{lem:manySourcesAtDecoder} studies the gain that can be obtained when all previously requested sources are stored at the decoder. Second,  Theorem~\ref{th:MRA} studies MRA without the  assumption of sequential access to the data and shows that both MRA and Sequential MRA achieve the same rate-storage region.

\begin{definition}[Family of subsets of previous requests] Let $k$ denote the current request.
A \emph{family of subsets of previous requests} $\Ffamk=\{\Ec_{1},\ldots, \Ec_{\Mk} \} $  is {a family of subsets} of the set $\lb 0, L \rb /\{k\}$, where each subset is a  set of previous requests that might be available at the decoder. $\Mk$ stands for the number of possible subsets available at the decoder.
%When many sources may be available at the decoder, (and not only one as in Definition~\ref{def:MRA}), $\Ffamk=\{\Ec_{1},\ldots, \Ec_{\Mk} \} $  is \emph{a family of subsets} of the set $\lb 0, L \rb /\{k\}$. Each subset is a  set of previous requests that might be available at the decoder.
\label{def:FamilyPreviousRequests}
\end{definition}

\textbf{Example}. To illustrate the definition of $\Ffamk$ (in Definition~\ref{def:FamilyPreviousRequests}) on a simple example, let us consider the directed graph in Figure~\ref{fig:ExGraph}. Here, $\Fc_{(2)}=\{\{0\}, \{0,1\}\}$, and  $\Fc_{(3)}=\{ \{0,1\},\{0,2\}, \{0,1,2\}\}$.
Note that the graph is directed giving rise to ordered sequences, but the family specifies set without any order, as the order does not matter in the conditional entropy. Therefore different paths in the directed graph may lead to the same subset in $\Ffamk$. Figure~\ref{fig:ExGraph}  shows such an example. The set of possible paths arriving in $3$ is $\{(0,1,3), (0,2,3), (0,1,2,3), (0,2,1,3)\}$, and contains 4 sequences ending with $(3)$, whereas the corresponding set  of subsets is $\Fc_{(3)}=\{ \{0,1\},\{0,2\}, \{0,1,2\}\}$, and contains only 3 subsets: the two sequences $(0,1,2,3), (0,2,1,3)$ are associated to the same subset $\{0,1,2\}$.



\begin{lemma}[Sequential MRA while storing {\sc all} the previously requested sources at the decoder]
Let $\{\Xl\}_{1\le l \le L}$ be a set of $L$ discrete i.i.d. sources (Definition~\ref{def:iidSources})  accessed under the Sequential MRA paradigm (Definition~\ref{def:SMRA}). Let us assume that {\sc all} the previously requested sources are stored  at the decoder. Let $k$ denote the current request,  $\Jsetk$ the set of possible previous requests (Definition~\ref{def:MRA}), and $\Ffamk=\{\Ec_{1},\ldots, \Ec_{|\Ffamk|} \} $  a family of subsets of previous requests (Definition~\ref{def:FamilyPreviousRequests}).

Assume that all statistics of the sources  are known by both the encoder and the decoder. 
Further assume that the number of possible previous request sets  $|\Ffamk|$  is finite. %The necessary and sufficient conditions for the existence of a vanishing-error-rate code  for lossless compression of the source $\Xk$ are:
The achievable rate-storage region  for lossless compression of the source $\Xk$ given the set of previously requested sources $X_{\Ejs}=\{\Xl\}_{l\in\Ejs}$ is:
\begin{subequations}
\begin{align}
\RkEjs &\ge H \left(  \Xk | X_{\Ejs} \right),   \\
\Sk&\ge \displaystyle \max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right).
\end{align}
\label{eq:RSmany}
\end{subequations}
Moreover, both storage and transmission costs are reduced when many previously requested sources are stored at the decoder:
\begin{subequations}
\begin{align}
 H \left(  \Xk | X_{\Ejs} \right) & \le H \left(  \Xk | X_{(j^*)} \right) ,   \\
\max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right) & \le \max_{j \in \Jsetk} H \left(  \Xk | \Xj \right).
%\RkEjs & \le\Rkjs ,   \\
%\max_{1\le j \le \Mk} H \left(  \Xk | X_{\Ec_{j}} \right) & \le \max_{j \in \Jsetk} H \left(  \Xk | \Xj \right).
\end{align}
\label{eq:RS1vsmany}
\end{subequations}
where $j^* \in \Ejs$ is the request preceding $k$. Equality in (\ref{eq:RS1vsmany}a)   and (\ref{eq:RS1vsmany}b) occurs if all  
the nodes of the one-hop neighborhood $\Jsetk$ are all connected to the initial node $0$.
\label{lem:manySourcesAtDecoder}
\end{lemma}

% \Sk&\ge \displaystyle \max_{j \in \Jsetk} H \left(  \Xk | \Xj \right)
%\label{eq:RS}
%\label{th:iid_stat_known}

\textbf{Remark}. Lemma~\ref{lem:manySourcesAtDecoder} allows to compare the case where a source is requested, while another (single) source $j^*$ is known at the decoder  (Theorem~\ref{th:iid_stat_known}), with the more general case of encoding along an arbitrary path of the navigation graph, where many sources $\Ejs$ might be available at the decoder (Lemma~\ref{lem:manySourcesAtDecoder}). Two conclusions can be drawn:\\
(i) As intuition suggests, taking into account more sources at the decoder, allows to reduce the rate at which $\Xk$ is transmitted   from $ H \left(  \Xk | X_{(j^*)} \right)$  to $ H \left(  \Xk | X_{\Ejs} \right)$.\\
(ii) More interestingly, the comparison of the achievable storage costs (\ref{eq:RS}b)   and  (\ref{eq:RSmany}b) done in  (\ref{eq:RS1vsmany}b) shows that a second counterintuitive conclusion can be drawn.
% Indeed, allowing to take into account more conditioning possibilities, will not  increase the storage cost. 
At first sight, one could expect that the maximum entropy storage should be bigger if we allow to store many sources at the decoder, since in Lemma~\ref{lem:manySourcesAtDecoder}, the maximum entropy for storage is taken over a bigger set $\Ffamk$ (\ref{eq:RSmany}b)  than in the case of a single previous request $\Jsetk$ (\ref{eq:RS}b).
However, since conditioning reduces entropy, we are able to show that even the storage cost can be reduced when many sources are available at the decoder. 
%Only primary sources, that can be requested first and therefore without any source available at the decoder, requires to be stored at their entropy rate  $ H \left(  \Xk \right)$. This is the only case, where an additional storage cost is required.

\begin{proof}[\textbf{\emph{Proof}}]
Let $Y$ be a sufficient statistic of $X_{\Ejs}$ for $\Xk$, such that 
%$X_{\Ejs} \to Y_{\js} \to \Xk$  builds a Markov chain. In particular, 
\begin{align}
H \left(  \Xk | Y \right)=H \left(  \Xk | X_{\Ejs} \right).
\label{eq:condEneq}
\end{align}
Let us apply Theorem~\ref{th:iid_stat_known} with $Y$ as the previous source available at the decoder.
Then, applying the conditional entropy equality \eqref{eq:condEneq}  leads to \eqref{eq:RSmany}.
%\begin{subequations}
%\begin{align}
%\RkEjs &\ge H \left(  \Xk | X_{\Ec_{j^*}} \right),   \\
%\Sk&\ge \displaystyle \max_{1\le j \le \Mk} H \left(  \Xk | X_{\Ec_{j}} \right).
%%\Sk&\ge \displaystyle \max_{j \in \Jsetk} H \left(  \Xk | \Xj \right),
% \end{align}
%\label{eq:boundH0}
%\end{subequations}

Note that, by applying Theorem~7,  we also construct, for each source of index $k$, a reordering of the  family of subsets of previous requests (Definition~\ref{def:FamilyPreviousRequests})  according to
\begin{align}
&\!\!\!\!\!  H (  \Xk | X_{\Ec_{1}} ) \le ...  \le H (  \Xk | X_{\Ec_{|\Ffamk|}} ).
\label{eq:orderSourcePreviousRequestSet}
\end{align}
%where $X_{\Ec_{1}}$ stands for the random vector with elements $X_i, i\in \Ec_{1}$.

%Case $\k$ is a primary source (See Definition~\ref{def:primarySource}). The source $\k$ can be requested first, while the decoder has not side information. Therefore, the set $\Ffamk$ contains the empty set, and $\max_{1\le j \le \Fk} H \left(  \Xk | X_{\Ec_{j}} \right)= H(\Xk) $,  since conditioning reduces entropy. 

%Case $\k$ is a not a primary source. 

We now show (\ref{eq:RS1vsmany}). By construction, the previously requested source $X_{(j^*)}$ belongs to the set of previously requested sources $X_{\Ejs}$. So, since conditioning reduces entropy, we have (\ref{eq:RS1vsmany}a).

Moreover, we have 
\begin{align}
 \forall \Ec \in \Ffamk, \forall l \in \Ec, H \left(  \Xk | X_{\Ec} \right) &\le  H \left(  \Xk | \Xl \right), 
 \label{eq:HsetH1}
\end{align}
which holds in particular for any source that belongs to $\Ec$ and to the one-hop neighborhood of $\Xk$, i.e. it holds for any source indexed by $l\in \Ec\cap\Jsetk$. Note that the set $\Ec\cap\Jsetk$ may contain many indexes since each set $\Ec$ corresponds to eventually many paths, as a path is ordered whereas the set is not. Finally, we get
\begin{align}
\max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right) &\le \max_{\Ec \in \Ffamk} \max_{l \in \Ec\cap\Jsetk} H \left(  \Xk | \Xl \right) \label{eq:upperboundHa}\\
&= \max_{l \in \Jsetk} H \left(  \Xk | \Xl \right) 
\label{eq:upperboundH}
\end{align}
where the second equality follows from the fact that $\cup_{\Ec \in \Ffamk} (\Ec\cap \Jsetk) = \Jsetk$ i.e. the multi-hop neighborhood of a node $k$ reduced to one-hop is exactly the  
one-hop neighborhood $\Jsetk$. This shows (\ref{eq:RS1vsmany}b).

{\em Case of equality in (\ref{eq:RS1vsmany}b)}. If the nodes of the one-hop neighborhood $\Jsetk$ are all connected to the initial node $0$ (meaning that the navigation can start at any source 
indexed by  $\Jsetk$), then there is equality in \eqref{eq:upperboundHa}  and therefore in  (\ref{eq:RS1vsmany}b). Note also that it is sufficient that the node in the one-hop neighborhood $\Jsetk$ that achieves the maximal entropy in \eqref{eq:upperboundH} can  be accessed directly (is connected to node $0$).
\end{proof}


\begin{theorem}[Simultaneous requests of many sources and optimality of  Sequential MRA] 
Let $\{\Xl\}_{1\le l \le L}$ be a set of $L$ discrete i.i.d. sources (Definition~\ref{def:iidSources}) accessed under the  MRA (Definition~\ref{def:MRA}) and the Sequential MRA (Definition~\ref{def:SMRA}) paradigms. Let  $\Kc \subset \lb 1, L \rb$ be a set of requests compatible with a given navigation graph, more precisely $\Kc$ contains the labels of a tree with root-node $0$. For each index $k\in \Kc$, let $\Ffamk $  be the family of subsets of previous requests (Definition~\ref{def:FamilyPreviousRequests}) that can describe all the paths in the navigation graph starting in $0$ and ending in $k$. 

Assume that all statistics of the sources  are known by both the encoder and the decoder and that the cardinality of $\Ffamk$ is finite. The achievable rate-storage region  for lossless compression of the source set $X_{\Kc}$ for MRA and Sequential MRA is:
\begin{subequations}
\begin{align}
R_\Kc &\ge  H(X_{\Kc})  \\
S_\Kc&\ge   \sum_{k \in \Kc} \max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right).
\end{align}
\label{eq:RS_MRAvsMRAnavig}
\end{subequations}
\label{th:MRA}
\end{theorem}
%\textbf{Remark}. Since Sequential MRA and MRA achieve the joint entropy at transmission, we conclude that interactivity is an additional service offered for free. 
%
\begin{proof}[\textbf{\emph{Proof}}] 
\emph{\textbf{Simultaneous requests and Sequential MRA}}. By definition of the set of requests $\Kc$, there exists at least one path in the navigation graph, whose labels are all in $\Kc$. Let $K=|\Kc|$ and let $(k_1,...,k_K)$ be such a path. Then, 
\begin{subequations}
\begin{align}
R_\Kc &= R_{(k_1)} + \sum_{i=1}^{K-1} R_{(k_{i+1})|(k_{1}... k_{i})}\\
&\ge H(X_{(k_1)})+\sum_{i=1}^{K-1} H(X_{(k_{i+1})}|X_{(k_{1})}... X_{(k_{i})})\\
&=  H(X_{\Kc})  \\
S_\Kc &= \sum_{k \in \Kc} \Sk \\
&\ge   \sum_{k \in \Kc} \max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right),
\end{align}
\label{eq:RSSMRAmultiple}
\end{subequations}
where (\ref{eq:RSSMRAmultiple}a) and (\ref{eq:RSSMRAmultiple}d) follow from the fact that the data are accessed sequentially in Sequential MRA, (\ref{eq:RSSMRAmultiple}b) and (\ref{eq:RSSMRAmultiple}e) follow from Lemma~\ref{lem:manySourcesAtDecoder} provided that the cardinality of $\Ffamk$ is finite, and (\ref{eq:RSSMRAmultiple}c) follows from the chain rule.

\emph{\textbf{Equivalence  of Sequential MRA and MRA}}. For a fair comparison, we assume that MRA is proposed under the same graph constraint as Sequential MRA.\\
\emph{Achievability}. The code built for  Sequential MRA (Theorem~\ref{th:iid_stat_known} and Lemma~\ref{lem:manySourcesAtDecoder}) can be used for MRA as well. Therefore, the same rate-storage region can be achieved.\\
\emph{Converse}.  Here, we use the converse of less stringent theorems, where more information is available at the encoder and/or decoder.\\
$\bullet \  \forall k\in \Kc, \forall \Ec \in \Ffamk, R_{\k | \Ec} \ge H \left(  \Xk | X_{\Ec} \right)$. Proof by contradiction, by invoking the converse of the Slepian-Wolf theorem \cite{Slepian73IT}
 with perfectly known side information statistics at the encoder. \\
$\bullet \  \forall k\in \Kc, \Sk \ge  \max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right)$. Proof by contradiction. If $\Sk <  \max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right),$  then with non zero probability, the side information might be $X_{\Ec^\dagger}$, where $\Ec^\dagger = \arg  \max_{\Ec \in \Ffamk} H \left(  \Xk | X_{\Ec} \right)$.  From the converse of the Slepian Wolf theorem \cite{Slepian73IT}, the source $\Xk$ can not be recovered at the decoder.
\end{proof}

\textbf{Summary of results}. Theorem~\ref{th:MRA} draws the general conclusion of all the theorems derived in Sections~\ref{sec:RSbounds:iid}
and~\ref{sec:RSboundsMRA:iid} related to discrete i.i.d. but correlated sources. Indeed, the conclusions are threefold.\\
(i) in order to build a massive random access scheme, one can assume, without loss of optimality, that the sources are requested one after the other (equivalence of MRA and  Sequential MRA),\\
(ii) massive random access  can be achieved without any loss in terms of transmission rate. Indeed, the minimal transmission rate (\ref{eq:RS_MRAvsMRAnavig}a) is the same as if one could compress directly the requested sources \cite[Theorem 3.2.1]{cover2006b}.\\
(iii) the cost of  massive random access is in the storage only. Interestingly, and also counter-intuitively, the storage cost decreases with the memory allowed at the decoder.






